Multi-population Ensemble Genetic Programming via Cooperative Coevolution and Multi-view Learning for Classification

This paper introduces Multi-population Ensemble Genetic Programming (MEGP), a computational intelligence framework that integrates cooperative coevolution and the multiview learning paradigm to address classification challenges in high-dimensional and heterogeneous feature spaces. MEGP decomposes the input space into conditionally independent feature subsets, enabling multiple subpopulations to evolve in parallel while interacting through a dynamic ensemble-based fitness mechanism. Each individual encodes multiple genes whose outputs are aggregated via a differentiable softmax-based weighting layer, enhancing both model interpretability and adaptive decision fusion. A hybrid selection mechanism incorporating both isolated and ensemble-level fitness promotes inter-population cooperation while preserving intra-population diversity. This dual-level evolutionary dynamic facilitates structured search exploration and reduces premature convergence. Experimental evaluations across eight benchmark datasets demonstrate that MEGP consistently outperforms a baseline GP model in terms of convergence behavior and generalization performance. Comprehensive statistical analyses validate significant improvements in Log-Loss, Precision, Recall, F1 score, and AUC. MEGP also exhibits robust diversity retention and accelerated fitness gains throughout evolution, highlighting its effectiveness for scalable, ensemble-driven evolutionary learning. By unifying population-based optimization, multi-view representation learning, and cooperative coevolution, MEGP contributes a structurally adaptive and interpretable framework that advances emerging directions in evolutionary machine learning.

==> fig_calibration.tex <==

\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.32\textwidth}
  \includegraphics[width=\linewidth]{SST2G_Calibration.png}
  \caption{SST2G}\label{fig_cal_sst2g}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.32\textwidth}
  \includegraphics[width=\linewidth]{20NG_Calibration.png}
  \caption{20NG}\label{fig_cal_20ng}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.32\textwidth}
  \includegraphics[width=\linewidth]{MNIST_Calibration.png}
  \caption{MNIST}\label{fig_cal_mnist}
\end{subfigure}

\par\vspace{0.9em} % <-- add POSITIVE space between rows

\hspace{\fill}
\begin{subfigure}[t]{0.36\textwidth}
  \includegraphics[width=\linewidth]{CIFAR10_Calibration.png}
  \caption{CIFAR10}\label{fig_cal_cifar10}
\end{subfigure}
\hspace{0.02\textwidth}
\begin{subfigure}[t]{0.36\textwidth}
  \includegraphics[width=\linewidth]{MSC17_Calibration.png}
  \caption{MSC17}\label{fig_cal_msc17}
\end{subfigure}
\hspace{\fill}

\caption{Reliability diagrams (test) before (\textcolor{orange}{orange}) and after (\textcolor{blue}{blue}) temperature scaling. Each panel shows empirical accuracy vs.\ predicted confidence using 20 equal-width bins; empty bins omitted; probabilities clipped to \([\,\varepsilon,1-\varepsilon\,]\). The dashed line denotes perfect calibration; \(T\) fitted on validation and applied to test.}
\label{fig_calibration}
\end{figure*}





==> fig_histogram.tex <==

\begin{figure*}[ht]
\centering
\captionsetup[sub]{justification=centering}
% ---------- Row 1 (three panels) ----------
\begin{minipage}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{histogram_SST2G.png}
  \subcaption{SST2G}
  \label{subfig:hist_sst2g}
\end{minipage}\hfill
\begin{minipage}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{histogram_20NG.png}
  \subcaption{20NG}
  \label{subfig:hist_20ng}
\end{minipage}\hfill
\begin{minipage}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{histogram_MNIST.png}
  \subcaption{MNIST}
  \label{subfig:hist_mnist}
\end{minipage}

\vspace{0.8em} % small, safe vertical gap

% ---------- Row 2 (two centered panels) ----------
\begin{minipage}[b]{0.38\textwidth}
  \includegraphics[width=\linewidth]{histogram_CIFAR10.png}
  \subcaption{CIFAR10}
  \label{subfig:hist_cifar10}
\end{minipage}\hspace{0.02\textwidth}
\begin{minipage}[b]{0.38\textwidth}
  \includegraphics[width=\linewidth]{histogram_MSC17.png}
  \subcaption{MSC17}
  \label{subfig:hist_msc17}
\end{minipage}

\caption{Embedding-dimension usage across canonical logits. Bars show the frequency with which each embedding dimension appears in the canonical GP expressions for each dataset (sorted in descending order).}
\label{fig_histogram}
\end{figure*}


==> fig_importance.tex <==
\begin{figure*}[t]
  \centering

  % Row 1
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\linewidth]{SST2G_contribution_bars.png}
    \caption{SST2G}\label{fig_importance_sst2g}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\linewidth]{20NG_contribution_bars.png}
    \caption{20NG}\label{fig_importance_20ng}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\linewidth]{MNIST_contribution_bars.png}
    \caption{MNIST}\label{fig_importance_mnist}
  \end{subfigure}

  \vspace{0.35em}

  % Row 2 (centered pair)
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{CIFAR10_contribution_bars.png}
    \caption{CIFAR10}\label{fig_importance_cifar10}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{MSC17_contribution_bars.png}
    \caption{MSC17}\label{fig_importance_msc17}
  \end{subfigure}

  \caption{Top embedding dimensions by mean absolute contribution $\bar I_j$ for each dataset. Blue bars show $\bar I_j$; red whiskers annotate the share of runs in which the dimension appears (and the expected count).}
  \label{fig_importance}
\end{figure*}



==> fig_metrics.tex <==

\begin{figure*}[t]
\centering
% -------- Row 1 --------
\subfloat[AUC]{%
  \includegraphics[width=0.32\textwidth]{AUC.png}%
  \label{fig:metric_auc}}
\hfill
\subfloat[Brier score]{%
  \includegraphics[width=0.32\textwidth]{Brier.png}%
  \label{fig:metric_brier}}
\hfill
\subfloat[Complexity]{%
  \includegraphics[width=0.32\textwidth]{Complexity.png}%
  \label{fig:metric_complexity}}

\vspace{0.7em}

% -------- Row 2 --------
\subfloat[ECE]{%
  \includegraphics[width=0.32\textwidth]{ECE.png}%
  \label{fig:metric_ece}}
\hfill
\subfloat[$F_1$ score]{%
  \includegraphics[width=0.32\textwidth]{F1_Score.png}%
  \label{fig:metric_f1}}
\hfill
\subfloat[Log-loss]{%
  \includegraphics[width=0.32\textwidth]{Log_Loss.png}%
  \label{fig:metric_logloss}}

\caption{Performance metrics across 30 independent runs per dataset. Each panel shows a raincloud-style summary (violin, box, and jittered points) for: (a) AUC, (b) Brier score, (c) complexity, (d) ECE, (e) $F_1$ score, and (f) log-loss. Dashed red lines depict means; boxes show medians and interquartile ranges.}
\label{fig_metrics}
\end{figure*}



==> fig_pdp_ale.tex <==

\begin{figure*}[t]
\centering
\captionsetup[subfigure]{justification=centering,labelformat=parens,aboveskip=2pt,belowskip=0pt}
% -------- Row 1: SST2G (3) + 20NG (2)
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{SST2G_d112_PDP_ALE.png}
\caption{SST2G, $d_{112}$}\label{subfig:pdpale_sst2g_d112}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{SST2G_d459_PDP_ALE.png}
\caption{SST2G, $d_{459}$}\label{subfig:pdpale_sst2g_d459}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{SST2G_d687_PDP_ALE.png}
\caption{SST2G, $d_{687}$}\label{subfig:pdpale_sst2g_d687}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{20NG_d112_PDP_ALE.png}
\caption{20NG, $d_{112}$}\label{subfig:pdpale_20ng_d112}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{20NG_d687_PDP_ALE.png}
\caption{20NG, $d_{687}$}\label{subfig:pdpale_20ng_d687}
\end{subfigure}

\vspace{0.35em}

% -------- Row 2: 20NG (1) + MNIST (3) + CIFAR10 (1)
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{20NG_d700_PDP_ALE.png}
\caption{20NG, $d_{700}$}\label{subfig:pdpale_20ng_d700}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{MNIST_d303_PDP_ALE.png}
\caption{MNIST, $d_{303}$}\label{subfig:pdpale_mnist_d303}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{MNIST_d618_PDP_ALE.png}
\caption{MNIST, $d_{618}$}\label{subfig:pdpale_mnist_d618}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{MNIST_d782_PDP_ALE.png}
\caption{MNIST, $d_{782}$}\label{subfig:pdpale_mnist_d782}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{CIFAR10_d404_PDP_ALE.png}
\caption{CIFAR10, $d_{404}$}\label{subfig:pdpale_cifar10_d404}
\end{subfigure}

\vspace{0.35em}

% -------- Row 3: CIFAR10 (2) + MSC17 (3)
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{CIFAR10_d721_PDP_ALE.png}
\caption{CIFAR10, $d_{721}$}\label{subfig:pdpale_cifar10_d721}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{CIFAR10_d812_PDP_ALE.png}
\caption{CIFAR10, $d_{812}$}\label{subfig:pdpale_cifar10_d812}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{MSC17_d400_PDP_ALE.png}
\caption{MSC17, $d_{400}$}\label{subfig:pdpale_msc17_d400}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{MSC17_d800_PDP_ALE.png}
\caption{MSC17, $d_{800}$}\label{subfig:pdpale_msc17_d800}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.19\textwidth}\centering
\includegraphics[width=\linewidth]{MSC17_d1100_PDP_ALE.png}
\caption{MSC17, $d_{1100}$}\label{subfig:pdpale_msc17_d1100}
\end{subfigure}

\caption{PDP/ALE summaries for selected embedding dimensions across datasets. Each panel shows the partial dependence of the predicted class probability (left within image) and the centered ALE with a $95\%$ CI band (right). PDP annotations report $\Delta p$; ALE annotations give $\int |{\rm ALE}|\,dx$. Panels are grouped by dataset.}
\label{fig_pdp_ale}
\end{figure*}



==> fig_scatters.tex <==

\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.32\textwidth}
  \includegraphics[width=\linewidth]{canonical_scatter_SST2G.png}
  \caption{SST2G}\label{fig_scatter_sst2g}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.32\textwidth}
  \includegraphics[width=\linewidth]{canonical_scatter_20NG.png}
  \caption{20NG}\label{fig_scatter_20ng}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.32\textwidth}
  \includegraphics[width=\linewidth]{canonical_scatter_MNIST.png}
  \caption{MNIST}\label{fig_scatter_mnist}
\end{subfigure}

\par\vspace{0.9em}

\hspace{\fill}
\begin{subfigure}[t]{0.36\textwidth}
  \includegraphics[width=\linewidth]{canonical_scatter_CIFAR10.png}
  \caption{CIFAR10}\label{fig_scatter_cifar10}
\end{subfigure}
\hspace{0.02\textwidth}
\begin{subfigure}[t]{0.36\textwidth}
  \includegraphics[width=\linewidth]{canonical_scatter_MSC17.png}
  \caption{MSC17}\label{fig_scatter_msc17}
\end{subfigure}
\hspace{\fill}

\caption{Canonical model selection: validation \(F_1\) vs.\ model complexity across 30 runs per dataset (SST2G, 20NG, MNIST, CIFAR10, MSC17). The dashed line marks the 1-SE threshold; red points indicate models within 1-SE of the best \(F_1\), with the chosen canonical model highlighted.}
\label{fig_scatters}
\end{figure*}



==> fig_upset.tex <==
% Requires in preamble:
% \usepackage{graphicx}
% \usepackage{subcaption}


\begin{figure*}[ht]
\centering

\captionsetup[subfigure]{justification=centering,singlelinecheck=false,font=small}

% ---- Top row (3 panels; fixed height) ----
\begin{subfigure}[t]{0.32\textwidth}
  \centering
  \includegraphics[height=0.22\textheight,keepaspectratio]{upset_plot_SST2G.png}
  \caption{SST2G}\label{fig_upset_sst2g}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.32\textwidth}
  \centering
  \includegraphics[height=0.22\textheight,keepaspectratio]{upset_plot_20NG.png}
  \caption{20NG}\label{fig_upset_20ng}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.32\textwidth}
  \centering
  \includegraphics[height=0.22\textheight,keepaspectratio]{upset_plot_MNIST.png}
  \caption{MNIST}\label{fig_upset_mnist}
\end{subfigure}

\vspace{0.6em}

% ---- Bottom row (2 centered panels; same height) ----
\begin{subfigure}[t]{0.46\textwidth}
  \centering
  \includegraphics[height=0.24\textheight,keepaspectratio]{upset_plot_CIFAR10.png}
  \caption{CIFAR10}\label{fig_upset_cifar10}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.46\textwidth}
  \centering
  \includegraphics[height=0.24\textheight,keepaspectratio]{upset_plot_MSC17.png}
  \caption{MSC17}\label{fig_upset_msc17}
\end{subfigure}

\caption{UpSet plots of embedding–dimension usage overlap for the canonical GP logits in each dataset. Bars (top) show intersection sizes; connected dots (bottom) indicate the participating logits for each intersection; left bars give total dimensions used by each logit.}
\label{fig_upset}
\end{figure*}



==> tab_datasets.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Datasets used in this study.}
\label{tab_datasets}
\begin{tabular}{l|l l l c c}
\hline
\textbf{Dataset} & \textbf{Modality} & \textbf{Task} &
\textbf{Records (train / val / test)} & \textbf{\#Cls} & \textbf{Official val?} \\
\hline
SST-2 GLUE (SST2G)             & Text       & Sentiment (binary)   & 67{,}349 / 872 / 1{,}821                 & 2  & Yes \\
20 Newsgroups (20NG)$^{\ast}$  & Text       & Topic                & 10{,}183 / 1{,}131$^{\ast}$ / 7{,}532    & 20 & No  \\
MNIST (MNIST)$^{\ast}$         & Image      & Digit classification & 54{,}000 / 6{,}000$^{\ast}$ / 10{,}000   & 10 & No  \\
CIFAR-10 (CIFAR10)$^{\ast}$    & Image      & Image classification & 45{,}000 / 5{,}000$^{\ast}$ / 10{,}000   & 10 & No  \\
MS COCO 2017 (MSC17)$^{\dagger}$ & Image+Text & Binary match         & 1{,}064{,}580$^{\dagger}$ / 118{,}290$^{\dagger}$ / 50{,}000$^{\dagger}$ & 2 & Yes (images) \\
\hline
\end{tabular}

\vspace{4pt}
\begin{minipage}{0.96\textwidth}\footnotesize
\emph{Notes.}\\
$^{\ast}$ No official validation split; we hold out 10\% of the training set for validation.\\
$^{\dagger}$ Counts are at the \emph{pair} level for image–caption matching (each positive caption paired with one hard negative; 1:1). Because \texttt{test2017} lacks public labels, we test on \texttt{val2017} (5{,}000 images) and split \texttt{train2017} into train/val (106{,}458 / 11{,}829 images).
\end{minipage}
\end{table*}





==> tab_gp_parameters.tex <==

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Genetic Programming (GP) configuration used in this study.}
\label{tab_gp_parameters}
\begin{tabular}{l|l}
\hline
\textbf{Parameter} & \textbf{Value} \\
\hline
Number of runs & 30 \\
Number of populations & Equal to the constructed views \\
Population size & 30 \\
Max generations & 150 \\
Stall generations & 30 \\
Genes per individual & 10 \\
Max tree depth & 10 \\
Initialization & Half-and-Half \\
$EF^{\mathrm{iso}}$ & 0.033 \\
$EF^{\mathrm{en}}$ & 0.10 \\
$p_{\mathrm{en}}$ & 0.75 \\
$p_c$ (crossover) & 0.84 \\
$p_m$ (mutation) & 0.14 \\
$p_r$ (reproduction) & 0.02 \\
Constant range & $[-10,\,10]$ \\
Functional nodes & $+,\,-,\,/,\times$ \\
Batch size & data size / 50 \\
Epochs & 1000 \\
Learning rate & 0.001 \\
\hline
\end{tabular}
\end{table}



==> tab_metric_results.tex <==

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Mean $\pm$ 95\% CI (t$_{29}$) over 30 runs per dataset and metric.}
\label{tab_metric_results}
\begin{tabular}{l|cccccc}
\hline
\textbf{Dataset} & $\mathbf{F_1}$ & \textbf{AUC} & \textbf{ECE} & \textbf{Brier} & \textbf{Log-Loss} & \textbf{Complexity} \\
\hline
SST2G   & 0.950 $\pm$ 0.008 & 0.950 $\pm$ 0.003 & 0.022 $\pm$ 0.002 & 0.061 $\pm$ 0.005 & 0.179 $\pm$ 0.021 & 15{,}316 $\pm$ 513 \\
20NG    & 0.776 $\pm$ 0.006 & 0.878 $\pm$ 0.015 & 0.068 $\pm$ 0.003 & 0.155 $\pm$ 0.006 & 0.667 $\pm$ 0.014 & 25{,}137 $\pm$ 1{,}048 \\
MNIST   & 0.982 $\pm$ 0.004 & 0.963 $\pm$ 0.002 & 0.025 $\pm$ 0.002 & 0.039 $\pm$ 0.002 & 0.107 $\pm$ 0.005 & 1{,}107 $\pm$ 62 \\
CIFAR10 & 0.973 $\pm$ 0.007 & 0.960 $\pm$ 0.007 & 0.027 $\pm$ 0.002 & 0.042 $\pm$ 0.002 & 0.104 $\pm$ 0.006 & 47{,}740 $\pm$ 1{,}469 \\
MSC17   & 0.973 $\pm$ 0.006 & 0.950 $\pm$ 0.006 & 0.032 $\pm$ 0.002 & 0.048 $\pm$ 0.003 & 0.109 $\pm$ 0.007 & 54{,}531 $\pm$ 2{,}250 \\
\hline
\end{tabular}
\end{table*}



==> tab_spfp.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Results of the SPFP procedure executed on the \emph{training set}. For each dataset we report the embedding dimension $d$, the number of views, the total number of selected features (mean $\pm$ s.d.), and the per-view allocation.}
\label{tab_spfp}
\begin{tabular}{l|c c c l}
\hline
\textbf{Dataset} & \textbf{Embedding Dimensions} & \textbf{\# Views} & \textbf{\#Features} & \textbf{Dimensions per View} \\
\hline
SST2G   & 768  & 4 & $192 \pm 8.5$    & \{178, 195, 201, 194\} \\
20NG    & 768  & 3 & $256 \pm 16.5$   & \{233, 264, 271\} \\
MNIST   & 1024 & 4 & $256 \pm 25.4$   & \{220, 251, 262, 291\} \\
CIFAR10 & 1024 & 5 & $204.8 \pm 19.5$ & \{181, 190, 199, 220, 234\} \\
MSC17   & 1152 & 4 & $288 \pm 24.7$   & \{254, 282, 293, 323\} \\
\hline
\end{tabular}
\end{table*}



==> tab_symbol_stats.tex <==
\begin{table*}[t]
\centering
\footnotesize
\caption{Symbol usage, sparsity, and complexity of canonical GP logits.}
\label{tab_symbol_stats}
\begin{tabular}{l|rrrrrrrrrrrr}
\hline
\textbf{Dataset} & \textbf{\#Logits} & \textbf{Unique D} & \textbf{M D/L} & \textbf{M Nodes} & \textbf{M Depth} & \textbf{M Consts/L} & \textbf{M Complexity} & \textbf{ops ($+$)} & \textbf{ops ($-$)} & \textbf{(ops $\times$)} & \textbf{ops ($\div$)} \\
\hline
SST2G   & 2  & 31  & 21.00 & 70  & 27 & 1.00 & 1007 & 15  & 15  & 13  & 13  \\
20NG    & 20 & 113 & 19.00 & 109 & 24 & 2.00 & 1298 & 236 & 231 & 202 & 200 \\
MNIST   & 10 & 17  & 4.00  & 15  & 6  & 1.00 & 62   & 21  & 19  & 10  & 10  \\
CIFAR10 & 10 & 76  & 12.50 & 164 & 27 & 3.00 & 1954 & 182 & 170 & 151 & 150 \\
MSC17   & 2  & 34  & 19.00 & 270 & 33 & 5.00 & 3903 & 61  & 59  & 49  & 50  \\
\hline
\end{tabular}

\vspace{2pt}
\begin{minipage}{0.96\textwidth}\footnotesize
\textbf{Notes.} Abbreviations: \textbf{D} = embedding \emph{dimension}; \textbf{M} = \emph{median} across logits; \textbf{D/L} = \emph{dimensions per logit} (median). 
“\textbf{Unique D}” is the number of distinct embedding dimensions referenced by any canonical logit for that dataset. 
“\textbf{Total ops} ($\pm,\times,\div$)” are \emph{totals across all logits}. 
\textbf{M Complexity} follows our GP measure used throughout (sum of function/terminal nodes with subtree accounting).
\end{minipage}
\end{table*}



==> tab_temp_scaling.tex <==

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Canonical GP models: test-set metrics before vs.\ after temperature scaling (\(T\) learned on validation, applied to test). \(F_1\) and AUC are unchanged by calibration.}
\label{tab_temp_scaling}
\begin{tabular}{l|ccccccc}
\hline
\textbf{Dataset} & $\mathbf{F_1}$ & \textbf{AUC} & \textbf{Complexity} & \textbf{Log-Loss (pre $\Rightarrow$ post)} & \textbf{Brier (pre $\Rightarrow$ post)} & \textbf{ECE (pre $\Rightarrow$ post)} & $\mathbf{T}$ \\
\hline
SST2G   & 0.979 & 0.941 & 12{,}642 & $0.092 \Rightarrow 0.090$ & $0.054 \Rightarrow 0.049$ & $0.019 \Rightarrow 0.008$ & 1.10 \\
20NG    & 0.810 & 0.888 & 28{,}915 & $0.620 \Rightarrow 0.588$ & $0.136 \Rightarrow 0.129$ & $0.058 \Rightarrow 0.014$ & 1.85 \\
MNIST   & 0.991 & 0.964 & 867      & $0.120 \Rightarrow 0.115$ & $0.044 \Rightarrow 0.040$ & $0.029 \Rightarrow 0.010$ & 1.20 \\
CIFAR10 & 0.991 & 0.959 & 45{,}331 & $0.123 \Rightarrow 0.115$ & $0.038 \Rightarrow 0.037$ & $0.024 \Rightarrow 0.008$ & 1.25 \\
MSC17   & 0.991 & 0.933 & 46{,}881 & $0.103 \Rightarrow 0.101$ & $0.035 \Rightarrow 0.034$ & $0.022 \Rightarrow 0.009$ & 1.15 \\
\hline
\end{tabular}
\end{table*}



==> tab_top3_monotonicity.tex <==

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Top-3 features per dataset with importance, PDP/ALE monotonicity (|Spearman~$\rho$|), direction from PDP, and brief notes.}
\label{tap_top3_monotonicity}
\begin{tabular}{l|lccccl}
\hline
\textbf{Dataset} & \textbf{Dimension} & \textbf{Importance} & \textbf{PDP Monotonicity} & \textbf{ALE Monotonicity} & \textbf{Direction} & \textbf{Notes} \\
\hline
\multirow{3}{*}{\textbf{SST2G}}
 & d687 & 9.9965 & 0.99 & 1.00 & \(+\) (increasing) & dominant \\
 & d112 & 9.9440 & 0.99 & 1.00 & \( - \) (decreasing) & clean effect \\
 & d459 & 8.4562 & 0.49 & 0.64 & non-monotonic & nonlinear \\ \hline
\multirow{3}{*}{\textbf{20NG}}
 & d112 & 148.8794 & 0.99 & 1.00 & \(+\) (increasing) & dominant \\
 & d687 & 142.3586 & 0.99 & 1.00 & \( - \) (decreasing) & clean effect \\
 & d700 & 92.9763 & 0.58 & 0.16 & \( - \) (decreasing) & interaction/correlation; nonlinear \\ \hline
\multirow{3}{*}{\textbf{MNIST}}
 & d618 & 29.6173 & 1.00 & 1.00 & \(+\) (increasing) & dominant \\
 & d303 & 20.2911 & 0.99 & 1.00 & \( - \) (decreasing) & clean effect \\
 & d782 & 6.4715 & 0.60 & 0.53 & \( - \) (decreasing) & nonlinear \\ \hline
\multirow{3}{*}{\textbf{CIFAR10}}
 & d721 & 191.7574 & 0.99 & 1.00 & \(+\) (increasing) & dominant \\
 & d812 & 149.8946 & 0.96 & 0.99 & \( - \) (decreasing) & clean effect \\
 & d404 & 149.7377 & 0.71 & 0.96 & \( - \) (decreasing) & nonlinear \\ \hline
\multirow{3}{*}{\textbf{MSC17}}
 & d1100 & 60.5356 & 0.99 & 1.00 & \(+\) (increasing) & dominant \\
 & d400  & 51.9222 & 0.95 & 1.00 & \( - \) (decreasing) & clean effect \\
 & d800  & 47.6701 & 0.55 & 0.66 & \( - \) (decreasing) & nonlinear \\
\hline
\end{tabular}
\end{table*}



==> tab_transformer_characteristics.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Transformer backbones used in this study (all encoders are frozen).}
\label{tab_transformer_characteristics}
\begin{tabular}{l|l l l c l}
\hline
\textbf{Model} & \textbf{Modality} & \textbf{$d_{\mathrm{model}}$ / Layers / Heads} &
\textbf{Embedding to GP} & \textbf{Params (M)} \\
\hline
ModernBERT-base$^{\ast}$ & Text       & 768 / 22 / 12                  & 768  & 149  \\
DINOv2 ViT-L/14$^{\dagger}$ & Image    & 1024 / 24 / 16                 & 1024 & 300 \\
SigLIP So400M (p14-384)$^{\ddagger}$ & Image+Text & 1152 / 27 / 16 (both towers) & 1152 & 400 (total)\\
\hline
\end{tabular}

\vspace{4pt}
\begin{minipage}{0.96\textwidth}\footnotesize
\emph{Notes.}\\
$^{\ast}$ Variant/checkpoint: \texttt{answerdotai/ModernBERT-base}. Embedding: 768-D final-layer [CLS] token.\\
$^{\dagger}$ Variant/checkpoint: \texttt{facebook/dinov2-large} (\texttt{dinov2\_vitl14}). Embedding: 1024-D final [CLS]; inputs 224$\times$224; patch size 14.\\
$^{\ddagger}$ Variant/checkpoint: \texttt{google/siglip-so400m-patch14-384}. Embedding: 1152-D concatenation of 576-D image + 576-D text projected, unit-normalized features (first 576 image, second 576 text).\\
We standardize (z-score) non-normalized embeddings (ModernBERT, DINOv2) using training-set statistics; SigLIP embeddings remain unit-normalized.
\end{minipage}
\end{table*}


